Stabilizing Dynamical Systems via Policy Gradient Methods

Stabilizing an unknown control system is one of the most fundamental problems in control systems engineering. In this paper, we provide a simple, model-free algorithm for stabilizing fully observed dynamical systems. While model-free methods have become increasingly popular in practice due to their simplicity and flexibility, stabilization via direct policy search has received surprisingly little attention. Our algorithm proceeds by solving a series of discounted LQR problems, where the discount factor is gradually increased. We prove that this method efficiently recovers a stabilizing controller for linear systems, and for smooth, nonlinear systems within a neighborhood of their equilibria. Our approach overcomes a significant limitation of prior work, namely the need for a pre-given stabilizing control policy. We empirically evaluate the effectiveness of our approach on common control benchmarks.

==> body.tex <==













==> body/problem_statement.tex <==
\section{Preliminaries}
\subsection{Notation \& Problem Setup}
Given $\matx_0 \sim \mathcal{D}$ with $\E[\matx_0 \matx_0^\top] = $, the states evolve according to, $\matx_{t+1} = A\matx_t + B\matu_t.$


We consider the discounted problem over an infinite horizon, where the cost of a state feedback controller $K$ is defined as, 
\begin{align}
\label{eq:discounted_problem}
	J_K(\matx) = \sum_{t=0}^\infty \gamma^t \matx^\top(Q + K^\top R K) \matx.
\end{align}
We see that any state feedback controller $K$ for which the above objective is finite, satisfies the following Lyapunov equation:
\begin{align*}
	P_K= Q + K^\top R K + \gamma(A+BK)^\top P_K (A+BK).
\end{align*}
Therefore, for a controller $K$ to have finite cost it is necessary and sufficient that the operator $\sqrt{\gamma}(A+BK)$ is stable. Furthermore, we observe that as a potential initialization strategy for policy gradients, the controller $K=0$ is guaranteed to have finite cost for $\gamma = c \times \opnorm{A}^{-2}$ for any $c \in (0,1)$.

\subsection{Gradient computation}

Assume that $K$ is such that $\sqrt{\gamma}(A+BK)$ is stabilizing, then
\begin{align*}
	J_K(\matx) &= \matx^\top P_K \matx \\ 
		   &= \matx^\top(Q +K^\top R K) \matx + \gamma \cdot J\left( (A+BK)\matx\right)
\end{align*}
Therefore, using a similar computation as before we get that,
\begin{align*}
	\gradk J_{K}(\matx) &= 2 (RK + \gamma B^\top P_K (A+BK))  \sum_{t=0}^\infty\matx_t \matx_t^\top \gamma^t \\ 
	&=2 Y_K  \sum_{t=0}^\infty\matx_t \matx_t^\top \gamma^t,
\end{align*}
where $\{\matx_t\}_{t=0}^\infty$ is the sequence of states generated by the controller $K$ and $Y_{K} \defeq RK + \gamma B^\top P_K (A+BK)$.

\section{Smoothness \& Gradient Domination} 

We use a few of the helper lemmas also from the Fazel paper. Define the following,  
\begin{align}
J_{t,K}(\matx)  &= \gamma^t \cdot \matx^\top P_K \matx\\
Q_{t}(\matx, K \matx) &= \gamma^t \cdot \matx^\top(Q + K^\top RK)\matx  + \gamma^t \cdot J_{t+1,K}\left((A +BK)\matx \right) \\ 
A_{t,K} &= Q_{t}(\matx, K' \matx) - J_{t,K}(\matx) 
\end{align}
\begin{lemma}
Let $\{ (\matx_j', \matu_j')\}_{j=1}^H$ be the sequence of states and inputs generated by the controller $K'$. If $K$ and $K'$ both have finite costs, then, 
\begin{align}
\label{eq:cost_difference}
J_{K'}(\matx) - J_K(\matx) = \sum_{t=0}^\infty A_{t,K}(\matx_t', \matu_t')
\end{align}
Furthermore, 
\begin{align*}
A_{j,K}(\matx, K' \matx) &= \gamma^t \matx^\top (K' - K)^\top (\gamma B^\top P_{K}B + R)(K' -K)\matx 
+ 2\gamma^t \matx^\top(K'-K)^\top (RK + \gamma B^\top P_{K}(A+BK))\matx  \\ 
& = \gamma^t \matx^\top (K' - K)^\top (\gamma B^\top P_{K}B + R)(K' -K)\matx + 2\gamma^t \matx^\top(K'-K)^\top Y_K\matx \\
& \geq - \traceb{\matx\matx^\top Y_K^\top (R+\gamma B^\top P_K B)^{-1} Y_K}
\end{align*}
\end{lemma}
\begin{proof}
This is the analogue of Lemma 10, the cost difference lemma, for the discounted problem. The last inequality again follows from the analogous argument from Fazel et al found on pg 20 of their manuscript.
\end{proof}

\subsection{Gradient Domination}

Let $\Sigma_\star = \sum_{t=0}^\infty \gamma^t \matx_t^\star (\matx_t^\star)^\top$ where $\{\matx_t^\star\}_{t=0}^\infty$ is the sequence of states generated by the optimal controller. Let $\Sigma_K = \sum_{t=0} \gamma^t\matx_t \matx_t^\top$ be the discounted state covariance for the sequence of states generated under $K$. 

Then, by the exact argument from Fazel et al, 
\begin{align*}
J(K) - J(\Kst) \leq \frac{\opnorm{\Sigma_\star}}{\sigma_{\min}(\Sigma_K)^2 \sigma_{\min(R)}}\traceb{\gradk J(K)^\top \gradk J(K)} 
\end{align*}

\subsection{Almost Smoothness}

By the lemma above, 
\begin{align*}
	J_{K'}(\matx) - J_K(\matx) &= \sum_{t=0}^\infty A_{t,K}(\matx_t', \matu_t') \\
	&= \traceb{\left(\sum_{t=0}^\infty \gamma^t \matx_t' (\matx_t')^\top\right) (K'-K)^\top(R+\gamma B^\top P_K B)(K'-K)} 
	+ 2 \traceb{\left(\sum_{t=0}^\infty \gamma^t \matx_t' (\matx_t')^\top\right)(K'-K)^\top Y_K}
\end{align*}

\subsection{Thoughts}

Policy gradients should converge to the optimal solution on the discounted problem.

\newpage
\section{Increasing the Discount Factor}

Define $P^\star_{j}$ to be the optimal value function for the problem in \Cref{eq:discounted_problem} with discount factor $\gamma_j$. Furthermore, 
define 
\begin{align*}
J(K; \gamma) &\defeq \E \left[ \sum_{t=0}^\infty \gamma^t \cdot \matx_t^\top (Q + K^\top R K)\matx \right] \\
 &\text{s.t } \matx_{t+1} = (A + BK)\matx_t 
\end{align*}



\noindent Consider the following algorithm: 

\begin{itemize}
	\item Initialize $\gamma_0 = c \cdot \opnorm{A}^{-2}$ for some $c \in (0,1)$
	\item Set $R = I$ and $Q = ???$
	\item Using policy gradients initialized at $0$, compute the state feedback controller $\Kst$ which solves the discounted LQR problem with discount factor $\gamma_0$. 
	\item Return $\Kst$
\end{itemize}


\begin{proposition}
Assume that $Q \succ I$. Then, for all $j \geq 0$, it holds that
\begin{itemize}
	\item $\sqrt{\gamma_{j+1}}(A + BK_{j})
$ is a stable matrix 
\item $J(K_j; \gamma_{j+1}) < \infty$
\end{itemize}
\end{proposition}
\begin{proof}
 \end{proof}
\newpage
\section{Technical Lemmas}

\begin{fact}
A matrix $A$ is stable if and only if 
\begin{align*}
\lim_{t\rightarrow\infty} A^t = 0.
\end{align*}
\end{fact}








